Band tilt induced nonlinear Nernst effect in topological insulators: An efficient generation of high-performance spin polarization

Topological insulators (TIs) hold promise as a platform for spintronics applications due to the fascinating spin-momentum locking (SML) of the surface states. One particular interest lies in using TIs as spin-polarized sources for spintronics structures. Here, we propose the band tilt induced nonlinear Nernst effect (NLNE) in TIs as a clean and efficient route to generate high-performance spin polarization (SP). We show that in the presence of SML and hexagonal warping effect a finite band tilt can induce an imbalance of two spin carriers and effectively give rise to spin-polarized NLNE current in TIs. In our scheme, both the spin current and charge current regime can be achieved under the thermal drive. The obtainable SP can be efficiently tuned in either a smooth or rapid way, exhibiting highly flexible tunability. In addition, near-unity SP can be generated within a wide range of tunable parameters, which is also found to be robust against temperature. Therefore, our work provides a mechanism to realize controllable room-temperature high-degree SP based on TIs, which is of essential importance for future spintronics applications.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );
 
        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );
 
        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
 
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
